ZDNS: A Fast DNS Toolkit for Internet Measurement

Active DNS measurement is fundamental to understanding and improving the DNS ecosystem. However, the absence of an extensible, high-performance, and easy-to-use DNS toolkit has limited both the reproducibility and coverage of DNS research. In this paper, we introduce ZDNS, a modular and open-source active DNS measurement framework optimized for large-scale research studies of DNS on the public Internet. We describe ZDNS' architecture, evaluate its performance, and present two case studies that highlight how the tool can be used to shed light on the operational complexities of DNS. We hope that ZDNS will enable researchers to better -- and in a more reproducible manner -- understand Internet behavior.

==> scraps.tex <==
Limitations and Future Work
% NB(dadrian): Sorry for the bad formatting, Overleaf doesn't have a line wrap functionality in its Vim mode. Kids these days don't even know how to write paper in Vim! No one wants to work anymore! All these grad students are quiet-quitting!

\textbf{TCP.}\quad
\zdns is capable of \textit{always} performing TCP resolutions, regardless of message size.
The TCP handshake causes a TCP-only bulk resolution takes longer than the equivalent UDP resolution on for commmon resolutions.
We did attempt a TCP-only resolution of all DNS names available in certificate transparency, and compared it to the same resolutions over UDP.
We found that sporadic network timeouts dominated the differences in resolutions between UDP and TCP.
We were unable to discern network unreliability and server uptime issues from differences caused by choice of L4.
This is an optimistic first result that indicates there is little availability difference between TCP and UDP for DNS.
More experimentation is required to confirm and characterize this initial observation.

% NB(dadrian): I ran this experiment in 2020 when we first thought about writing this paper, and determined that I couldn't get any actual results.

% Browsers, including Chrome~\cite{chrome-doh} and Firefox~\cite{firefox-doh}, recently added support for DoH, with Firefox defaulting to DoH in certain countries.
DoH establishes an HTTPS connection between the client and the server, and uses HTTP requests with the content type \texttt{application/dns-message} as a transport.
DoT establishes a TLS connection between the client and the server, but eschews the HTTP framing for the standard TCP framing for DNS messages.
% Both DoH and DoT provide transport security for DNS.
They do not attempt to provide the same authenticity guarantees as DNSSEC, which attempts to provide a chain of trust back to the root nameservers.
In order to support DoH and DoT, \zdns needs to embed a TLS library.
In both cases, \zdns will need to maintain TCP connections, which can affect performance due to the extra packets required to performance a TCP handshake, and since the UDP socket reuse optimization described in Section~\ref{sec:arch} is no longer possible.
However, in both DoH and DoT, \zdns may be able to reuse a TLS connection for multiple resolutions, depending on resolver behavior, which may mitigate the performance hit.
% NB(dadrian): Could probably delete these next two sentences.
The  library contains , which may be suitable for use with DNS.
If the extra state maintained by ZCrypto for measurement purposes causes too much of a performance impact, then \zdns could also consider using the Go Standard Library implementation of TLS.


\vspace{3pt} \noindent \textbf{Other Resolvers.}\quad
\zdns is a client and iterative resolver. It cannot be used to understand the behavior of other clients, nor the resolution behavior of other revolvers beyond what is observable by a single client. \zdns is not a server, nor is it Bind. However, DNS servers are a completely different type of software, so this is a reasonable limitation.
% NB(dadrian): Addressing comment that ZDNS could not be used to understand how Bind works, since they're different pieces of software.
% NB(dadrian): Can probably delete this section.

\todo{dadrian: Do we have any other limitations? If so, ping me on Slack and I'll write about them.}




CASE Study 2 (CAA)

%\begin{table}[]
%    \centering
%    \begin{tabular}{cr}
%    \toprule
%    \textbf{status} & \multicolumn{1}{c}{\textbf{\# of domains}} \\
%    \midrule
%    NOERROR & 64,203,223 \\
%    NXDOMAIN & 27,620,549 \\
%    SERVFAIL & 1,703,900 \\
%    REFUSED & 6,596 \\
%    ERROR & 7 \\
%    {\bf Total} & 93,534,275 \\
%    \bottomrule
%\end{tabular}
%\caption{CAA Case Study. Breakdown of query status for CAA records for $93M$
%domains on April 15th, 2022.\gakiwate{Drop table if need be.}}
%\label{tab:caa_casestudy_breakdown}
%\end{table}

% Next, we analyze the CAA features and configurations, if any, of $93M$
% domains measured using \zdns on April 15, 2022 over a period of roughly 4 hours.
% %Table~\ref{tab:caa_casestudy_breakdown} reports the breakdown of the returned
% %status. 
% Of the $93M$ domains queried, $64M$ domains returned a NOERROR code, $27M$
% returned an NXDOMAIN, while roughly $1.7M$ returned a SERVFAIL code, typically
% indicating lack of support for CAA records. The percentage breakdown of the
% query return status is near equal \ie, roughly 68\% of ccTLDs and gTLDs returned
% NOERROR while roughly 29\% returned NXDOMAIN.\gakiwate{simplify} We report on
% the results for these $64M$ domains and draw comparisons to results presented in
% Scheitle \etal from 2017~\cite{ccr2018_caa_first_look} wherever possible.

% Breakdown by TLDs
% \begin{table}[]
% \begin{tabular}{lrrr}
% \toprule
%  & \multicolumn{1}{c}{\textbf{gTLDs}} & \multicolumn{1}{c}{\textbf{ccTLDs}} & \multicolumn{1}{c}{\textbf{Total}} \\
% \midrule
% \textbf{Domains w/CAA} & 554844 & 527311 & 1082155 \\
% \textbf{(\% of NOERROR)} & 1.56\% & 1.85\% & 1.69\% \\
% \textbf{(\% of Total)} & 1.06\% & 1.27\% & 1.16\% \\
% \bottomrule
% \end{tabular}
% \caption{Breakdown of CAA enabled domains by TLD type.  Roughly $1.16\%$ of all
% domains are CAA enabled. ccTLDs have a slightly higher percentage of CAA
% enabled domains.
% }
% \end{table}

{\bf CAA Flag}. 
Another feature of the CAA record is the critical flag. The critical flag
prevents CAs from issuing certificates unless they recognize all the semantics
from the records. Roughly 15\% of the CAA enabled domains set the critical
flag. Fortunately, only 29 of these domains have invalid tags which would
prevent issuance of any certificates.

\begin{table}[]
\begin{tabular}{lr}
    \toprule
    \multicolumn{1}{c}{\textbf{CAA Tags}} & \multicolumn{1}{l}{\textbf{\# of Domains (\%)}} \\
    \midrule
    issue & 440117 (40.67\%) \\
    issuewild & 32308 (2.99\%) \\
    iodef & 647 (0.06\%) \\
    issue u iodef & 38114 (3.52\%) \\
    issuewild u iodef & 1384 (0.13\%) \\
    issue u issuewild & 535091 (49.45\%) \\
    issue u issuewild u iodef & 34035 (3.15\%) \\
    INVALID & 459 (0.04\%) \\
    \midrule
    {\bf Domains with CAA Records} & 1082155 (100\%) \\
    \bottomrule
\end{tabular}
\caption{Breakdown of the use of CAA Records by domains. Of the $64M$ domains
successfuly queried $1.08M$ domains (roughly 1.69\%) use CAA records. INVALID
combines non-standard tags. INVALID tags can lead to malformed DNS response
packets.}
\label{tab:caa_tags_breakdown}
\end{table}




Of CAA
enabled domains, we find  use the \dns{issue} tag, use the
\dns{issuewild} tag, and only 6.87\% use the \dns{iodef} tag. Roughly 50\%
of domains use both the \dns{issue} and \dns{issuewild} tags. The use of
\dns{iodef} tags is generally limited. Interestingly, we also
see 647 domains only use the \dns{iodef} tag.\footnote{A random sampling
suggests many domains are affiliated to Visa Inc. a financial services company.}
We find that some of the INVALID tags lead to malformed packets and may be a
result of incorrect input validation by a large registrar.\footnote{We have
reached out to the registrar and will report on any notable findings if any.}
\gakiwate{Messaged GoDaddy about this. Will see what they say}

Comparing to results from 2017, we see that the use of \dns{issue} tag has
remained largely stable, while the use of \dns{issuewild} has gone up from
25\% to 55.27\%. Perhaps most significant, is the drop of the use of \dns{iodef}
from 33\% of domains to only 6.87\% of domains~\cite[]{ccr2018_caa_first_look}.



%%%%%%%%%%%%%


\begin{table}[h!]
\begin{tabular}{lrr|rr}
    \toprule
    \multicolumn{1}{c}{\textbf{CA}} & \multicolumn{1}{c}{\textbf{issue}} & \multicolumn{1}{c}{\textbf{(\%)}} & \multicolumn{1}{c}{\textbf{issuewild}} & \multicolumn{1}{c}{\textbf{(\%)}} \\
    \midrule
    letsencrypt.org & 968714 & 92.47\% & 563633 & 93.48\% \\
    comodoca.com & 418701 & 39.97\% & 354224 & 58.75\% \\
    digicert.com & 385642 & 36.81\% & 360324 & 59.76\% \\
    globalsign.com & 256822 & 24.52\% & 249288 & 41.34\% \\
    certum.pl & 158689 & 15.15\% & 158032 & 26.21\% \\
    \bottomrule
    \end{tabular}
    \caption{Top~5 CA issuers for \dns{issue} and \dns{issuewild} tagged CAA records.
    \textnormal{Let's Encrypt is present in nearly all CAA records. \dns{certum.pl} is used primarily by \dns{.pl} domains.  We note that since domains may configure more than one CA, each column sums to more than 100\%. }}
    \label{tab:caa_issuers}
\end{table}

==> tables/massdns_v_alpha.tex <==
\begin{table}[h]
%\vspace{-5pt}
\centering
\small
\begin{tabular}{lllll}
\toprule
Lookup & Resolver & MassDNS & Alpha& Alpha\\ 
 & &  \% Success & \% Success &  Speed-up  \\ 
\midrule
A & Google &  12\% $\pm$ 2.5\% &  97.3\%  $\pm$ 0.05\% & 2.19x \\
A & Cloudflare  & 58\% $\pm$ 1.7\% & 98.2\%  $\pm$ 0.7\% & 0.81x \\
PTR & Google & 8.7\% $\pm$ 2\% & 88\% $\pm$ 0.1\% & 5.7x \\
PTR & Cloudflare  & 60\% $\pm$ 0.5\% & 90.5\% $\pm$ 0.1\%  & 0.98x \\
\bottomrule
\end{tabular}
\caption{
MassDNS vs \zdns: \textnormal{At best, \zdns successfully resolves 10~times more IPv4 addresses while achieving a 5.7~times performance speed-up.}}

\label{table:mass_alpha}
\end{table}



%Google, 

%peak instant performance is 50K
% --socket-count 500 -r google_resolver.txt -t A --processes 24 --hashmap-size 10000
%20.55PPS!

% after a great parameter tuning effort, we discover that  unintuitively, 
% adding less total sockets than hashmap-size decreases performance and using more sockets slows it down.


